Fast Virtual Gate Extraction For Silicon Quantum Dot Devices

Silicon quantum dot devices stand as promising candidates for large-scale quantum computing due to their extended coherence times, compact size, and recent experimental demonstrations of sizable qubit arrays. Despite the great potential, controlling these arrays remains a significant challenge. This paper introduces a new virtual gate extraction method to quickly establish orthogonal control on the potentials for individual quantum dots. Leveraging insights from the device physics, the proposed approach significantly reduces the experimental overhead by focusing on crucial regions around charge state transition. Furthermore, by employing an efficient voltage sweeping method, we can efficiently pinpoint these charge state transition lines and filter out erroneous points. Experimental evaluation using real quantum dot chip datasets demonstrates a substantial 5.84x to 19.34x speedup over conventional methods, thereby showcasing promising prospects for accelerating the scaling of silicon spin qubit devices.

==> tex/6-Conclusion.tex <==
\section{Conclusion}
Due to the overhead of obtaining a charge stability diagram, extracting a virtual gate without relying on the complete diagram is advantageous for large-scale quantum dot devices. To this end, we propose a search heuristic that probes a small subset of points near the charge transition lines for virtual gate extraction. The search heuristic results in an order of magnitude speedup in total runtime compared to the method that relies on a full charge stability diagram.
